Ruitenburg's Theorem via Duality and Bounded Bisimulations

For a given intuitionistic propositional formula A and a propositional variable x occurring in it, define the infinite sequence of formulae { A \_i | i$\ge$1} by letting A\_1 be A and A\_{i+1} be A(A\_i/x). Ruitenburg's Theorem [8] says that the sequence { A \_i } (modulo logical equivalence) is ultimately periodic with period 2, i.e. there is N $\ge$ 0 such that A N+2 $\leftrightarrow$ A N is provable in intuitionistic propositional calculus. We give a semantic proof of this theorem, using duality techniques and bounded bisimulations ranks.

==> Macro.tex <==
\RequirePackage{amsmath}
\newcommand{\cal}[1]{\mathcal{#1}}
\RequirePackage{amsthm}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}[proposition]{Theorem}
\newtheorem{lemma}[proposition]{Lemma}
\newtheorem{corollary}[proposition]{Corollary}

\RequirePackage[all]{xy}


\newcommand{\mcmt}{{\sc mcmt}\xspace}
\newcommand{\mcmtd}{$\text{\sc mcmt}^2$\xspace}
\newcommand{\tran}[1]{\ensuremath{\buildrel #1\over\longleftarrow}}
\newcommand{\arco}[1]{\ensuremath{\buildrel #1\over\longrightarrow}}
\newcommand{\arcos}[1]{\ensuremath{\buildrel #1\over\longrightarrow_+}}
\newcommand{\model}{\ensuremath{\zeta}\xspace}

\newcommand{\diff}{\ensuremath{\mathtt{diff}}}
\newcommand{\ARRAY}{\ensuremath{\mathtt{ARRAY}}\xspace}
\newcommand{\INDEX}{\ensuremath{\mathtt{INDEX}}\xspace}
\newcommand{\ELEM}{\ensuremath{\mathtt{ELEM}}\xspace}
\newcommand{\formulae}{formul\ae\xspace}
\newcommand{\unc}{\ensuremath{v}\xspace}
\newcommand{\fresh}{\ensuremath{z}\xspace}
\newcommand{\EQSYMBOL}{=}
\newcommand{\TILDE}{\sim}
\newcommand{\TARRAY}{\ensuremath{\ARRAY^{\TILDE}}}
\newcommand{\EQINDEX}{\ensuremath{\INDEX^{\EQSYMBOL}}}
\newcommand{\EQELEM}{\ensuremath{\ELEM^{\EQSYMBOL}}}
\newcommand{\EQARRAY}{\ensuremath{\ARRAY^{\EQSYMBOL}}}
\newcommand{\EQP}{\ensuremath{\mathcal{P}^{\EQSYMBOL}}}

\newcommand{\LRA}{\ensuremath{\mathcal{LRA}}\xspace}
\newcommand{\EUF}{\ensuremath{\mathcal{EUF}}\xspace}
\newcommand{\LIA}{\ensuremath{\mathcal{LIA}}\xspace}
\newcommand{\IDL}{\ensuremath{\mathcal{IDL}}\xspace}
\newcommand{\AX}{\ensuremath{\mathcal{AX}}\xspace}
\newcommand{\BAX}{\ensuremath{\mathcal{BAX}}\xspace}
\newcommand{\AXEXT}{\ensuremath{\mathcal{AX}_{{\rm ext}}}\xspace}
\newcommand{\AXDIFF}{\ensuremath{\AX_{\diff}}\xspace}
\newcommand{\T}{\ensuremath{\mathcal{T}}\xspace}

\newcommand{\clauseorange}[1]{\colorbox{yellow}{#1}}
\newcommand{\clausered}[1]{\colorbox{red}{#1}}
\newcommand{\clauseblue}[1]{\colorbox{blue}{\textcolor{white}{#1}}}
\newcommand{\clausegreen}[1]{\colorbox{green}{#1}}
\newcommand{\clausemagenta}[1]{\colorbox{magenta}{#1}}

\newcommand{\boxclause}[1]{\box{#1}}

\newcommand{\neglit}{\overline}

\newcommand{\Pivs}{s}
\newcommand{\Pivt}{t}
\newcommand{\Cthree}{E}
\newcommand{\Ctwo}{D}
\newcommand{\Cone}{C}

\newcommand{\s}[1]{\,#1\,}
\newcommand{\ds}[1]{\,\,\,#1\,\,\,}
\newcommand{\tfont}[1]{\mathit{#1}}

\newcommand{\showcite}[1]{\cite{#1}}
\newcommand{\todo}[1]{\fbox{\textcolor{red}{{\bf TODO}: #1}}}

\newcommand{\assign}{\ensuremath{:=}\xspace}

\newcommand{\bv}[2]{\ensuremath{{#1}_{[#2]}}}
\newcommand{\bitvector}{bit-vector\xspace}
\newcommand{\bitvectors}{bit-vectors\xspace}

\newcommand{\bvextr}[3]{\ensuremath{#1[#2:#3]}}
\newcommand{\bvconc}[2]{\ensuremath{#1\,::\,#2}}

\newcommand{\bvplus}[2]{\ensuremath{#1 + #2}}
\newcommand{\bvtimes}[2]{\ensuremath{#1 \cdot #2}}

\newcommand{\bvlt}[2]{\ensuremath{#1 < #2}}
\newcommand{\bvle}[2]{\ensuremath{#1 \leq #2}}

\newcommand{\bitand}[2]{\ensuremath{#1 \bitandsymb #2}}
\newcommand{\bitor}[2]{\ensuremath{#1 \bitorsymb #2}}
\newcommand{\bitnot}[1]{\ensuremath{\bitnotsymb #1}}

\newcommand{\bitandsymb}{\ensuremath{\&}}
\newcommand{\bitorsymb}{\ensuremath{|}}
\newcommand{\bitnotsymb}{\ensuremath{!}}

\newcommand{\tbv}{\ensuremath{\mathcal{BV}}\xspace}
\newcommand{\tbvc}{\ensuremath{\tbv_{C}}\xspace}
\newcommand{\tbva}{\ensuremath{\tbv_{A}}\xspace}
\newcommand{\tbvb}{\ensuremath{\tbv_{B}}\xspace}
\newcommand{\tbvcuf}{\ensuremath{(\tbv_{C}\cup\mathcal{UF})}\xspace}
\newcommand{\te}{\ensuremath{\mathcal{E}}\xspace}

\newcommand{\BVTerm}{\ensuremath{\tbv\mbox{-Term}}\xspace}
\newcommand{\BVTerms}{\ensuremath{\tbv\mbox{-Terms}}\xspace}
\newcommand{\BVAtom}{\ensuremath{\tbv\mbox{-Atom}}\xspace}
\newcommand{\BVAtoms}{\ensuremath{\tbv\mbox{-Atoms}}\xspace}
\newcommand{\BVLit}{\ensuremath{\tbv\mbox{-Literal}}\xspace}
\newcommand{\BVLits}{\ensuremath{\tbv\mbox{-Literals}}\xspace}

\newcommand{\TTerm}{\ensuremath{\T\mbox{-Term}}\xspace}
\newcommand{\TTerms}{\ensuremath{\T\mbox{-Terms}}\xspace}
\newcommand{\TAtom}{\ensuremath{\T\mbox{-Atom}}\xspace}
\newcommand{\BAtom}{\ensuremath{\mathcal{B}\mbox{-Atom}}\xspace}
\newcommand{\TAtoms}{\ensuremath{\T\mbox{-Atoms}}\xspace}
\newcommand{\TLit}{\ensuremath{\T\mbox{-Literal}}\xspace}
\newcommand{\TLits}{\ensuremath{\T\mbox{-Literals}}\xspace}
\newcommand{\TFormula}{\ensuremath{\T\mbox{-Formula}}\xspace}

\newcommand{\Tsolve}{\tsolver}
\newcommand{\tsolver}{\ensuremath{\mathcal{T}\mbox{-solver}}\xspace}
\newcommand{\tsolvers}{\ensuremath{\mathcal{T}\mbox{-solvers}}\xspace}
\newcommand{\bvsolver}{\ensuremath{\mathcal{BV}\mbox{-solver}}\xspace}
\newcommand{\bvsolvers}{\ensuremath{\mathcal{BV}\mbox{-solvers}}\xspace}
\newcommand{\eufsolver}{\ensuremath{\mathcal{EUF}\mbox{-solver}}\xspace}
\newcommand{\eufsolvers}{\ensuremath{\mathcal{EUF}\mbox{-solvers}}\xspace}
\newcommand{\dlsolver}{\ensuremath{\mathcal{DL}\mbox{-solver}}\xspace}
\newcommand{\dlsolvers}{\ensuremath{\mathcal{DL}\mbox{-solvers}}\xspace}
\newcommand{\smt}{SMT\xspace}
\newcommand{\smtt}{SMT\ensuremath{(\T)}\xspace}
\newcommand{\smteuf}{SMT\ensuremath{\mathit{(\euf)}}\xspace}
\newcommand{\smtbv}{SMT\ensuremath{\mathit{(\tbv)}}\xspace}
\newcommand{\smtdl}{SMT\ensuremath{\mathit{(\dl)}}\xspace}
\newcommand{\smtla}{SMT\ensuremath{\mathit{(\la)}}\xspace}
\newcommand{\smtlia}{SMT\ensuremath{\mathit{(\lia)}}\xspace}
\newcommand{\smtlra}{SMT\ensuremath{\mathit{(\lra)}}\xspace}
\newcommand{\smttt}[1]{SMT\ensuremath{(#1)}\xspace}
\newcommand{\smttonettwo}{SMT\ensuremath{(\tonetwo)}\xspace}
\newcommand{\dec}{Dec\xspace}
\newcommand{\dect}{Dec\ensuremath{(\T)}\xspace}
\newcommand{\decbv}{Dec\ensuremath{\mathit{(\tbv})}\xspace}
\newcommand{\declaint}{Dec\ensuremath{\mathit{(\laint)}}\xspace}
\newcommand{\dectt}[1]{Dec\ensuremath{(#1)}\xspace}
\newcommand{\dectonettwo}{Dec\ensuremath{(\tonetwo)}\xspace}
\newcommand{\DecT}[1]{\ensuremath{\mathit{Dec(}{#1}\mathit{)}}\xspace}
\newcommand{\DecTpos}[1]{\ensuremath{\mathit{Dec}^+\mathit{(}{#1}\mathit{)}}\xspace}

\newcommand{\DPe}[1]{\ensuremath{DP^=(#1)}}
\newcommand{\DP}[1]{\ensuremath{DP(#1)}}

\newcommand{\coarser}{\preceq}

\newcommand{\boolabs}[1]{\alpha(#1)}

\renewcommand{\iff}{\Leftrightarrow}
\newcommand{\imp}{\Rightarrow}
\newcommand{\range}[2]{\ensuremath{(0\le #1)\wedge (#1< 2^{#2})}}
\newcommand{\simplify}{{\sc Simplify}\xspace}
\newcommand{\opensmt}{{\sc OpenSMT}\xspace}
\newcommand{\opensmtcbe}{{\sc OpenSMT\_CBE}\xspace}
\newcommand{\opensmtbb}{{\sc OpenSMT\_BB}\xspace}
\newcommand{\mathsat}{{\sc MathSAT}\xspace}
\newcommand{\minisat}{{\sc MiniSAT}\xspace}
\newcommand{\cvctre}{{\sc CVC3}\xspace}
\newcommand{\yices}{{\sc Yices}\xspace}
\newcommand{\ztre}{{\sc Z3}\xspace}
\newcommand{\boolector}{{\sc Boolector}\xspace}
\newcommand{\beaver}{{\sc Beaver}\xspace}
\newcommand{\bat}{{\sc BAT}\xspace}
\newcommand{\spear}{{\sc Spear}\xspace}
\newcommand{\stp}{{\sc MathSAT}\xspace}

\newcommand{\bool}[1]{\ensuremath{\foltoprop(#1)}}

\newcommand{\BoolGen}[1]{\ensuremath{\mathsf{Bool+}{#1}}\xspace}
\newcommand{\BoolT}{\BoolGen{T}}
\newcommand{\proptofol}{\ensuremath{\mathit{Bool2\T}}\xspace}
\newcommand{\foltoprop}{\ensuremath{\T2Bool}\xspace}
\newcommand{\TsatisfiableGen}[1]{\ensuremath{{#1}\textit{-satisfiable}}\xspace}
\newcommand{\Tsatisfiable}{\TsatisfiableGen{T}}
\newcommand{\Psatisfiable}{\TsatisfiableGen{\mathsf{Bool}}}
\newcommand{\picktotalassign}{\ensuremath{\mathit{pick\_total\_assign}}\xspace}
\newcommand{\satres}{\ensuremath{\mathsf{sat}}\xspace}
\newcommand{\unsatres}{\ensuremath{\mathsf{unsat}}\xspace}
\newcommand{\analyzeconflict}{\ensuremath{\mathit{analyze\_conflict}}\xspace}
\newcommand{\analyzededuction}{\ensuremath{\mathit{deduce\&learn}}\xspace}
\newcommand{\backtrack}{\ensuremath{\mathit{backjump\&learn}}\xspace}
\newcommand{\learn}{\ensuremath{\mathit{learn}}\xspace}
\newcommand{\conflict}{\ensuremath{\pi^p}\xspace}
\newcommand{\deduction}{\ensuremath{\pi^p}\xspace}
\newcommand{\reasons}{\ensuremath{\Gamma^p}\xspace}
\newcommand{\currentstack}{\ensuremath{\beta^p}\xspace}
\newcommand{\currentinterp}{\ensuremath{\beta^p}\xspace}
\newcommand{\bcp}{\ensuremath{\textup{BCP}}\xspace}
\newcommand{\preprocess}{\ensuremath{\mathit{Preprocess}}\xspace}
\newcommand{\blevel}{\ensuremath{\mathit{no\_open\_branches}}\xspace}
\newcommand{\decidebranch}{\ensuremath{\mathit{decide\_new\_branch}}\xspace}
\newcommand{\cala}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\atoms}{\ensuremath{\mathit{Atoms}}}
\newcommand{\tatoms}{\ensuremath{\mathcal{T}\mbox{-atoms}}\xspace}
\newcommand{\tatom}{\ensuremath{\mathcal{T}\mbox{-atom}}\xspace}
\newcommand{\tlit}{\ensuremath{\mathcal{T}\mbox{-literal}}\xspace}
\newcommand{\tlits}{\ensuremath{\mathcal{T}\mbox{-literals}}\xspace}
\newcommand{\eufatoms}{\ensuremath{\mathcal{EUF}\mbox{-atoms}}\xspace}
\newcommand{\eufatom}{\ensuremath{\mathcal{EUF}\mbox{-atom}}\xspace}
\newcommand{\dlatoms}{\ensuremath{\mathcal{DL}\mbox{-atoms}}\xspace}
\newcommand{\dlatom}{\ensuremath{\mathcal{DL}\mbox{-atom}}\xspace}
\newcommand{\bvatoms}{\ensuremath{\mathcal{BV}\mbox{-atoms}}\xspace}
\newcommand{\bvatom}{\ensuremath{\mathcal{BV}\mbox{-atom}}\xspace}
\newcommand{\Tconsequence}{\ensuremath{\mathcal{T}\mbox{-consequence}}\xspace}
\newcommand{\Tconsequences}{\ensuremath{\mathcal{T}\mbox{-consequences}}\xspace}
\newcommand{\tconsequence}{\ensuremath{\mathcal{T}\mbox{-consequence}}\xspace}
\newcommand{\tconsequences}{\ensuremath{\mathcal{T}\mbox{-consequences}}\xspace}
\newcommand{\eufconsequence}{\ensuremath{\mathcal{EUF}\mbox{-consequence}}\xspace}
\newcommand{\eufconsequences}{\ensuremath{\mathcal{EUF}\mbox{-consequences}}\xspace}
\newcommand{\dlconsequence}{\ensuremath{\mathcal{DL}\mbox{-consequence}}\xspace}
\newcommand{\dlconsequences}{\ensuremath{\mathcal{DL}\mbox{-consequences}}\xspace}
\newcommand{\bvconsequence}{\ensuremath{\mathcal{BV}\mbox{-consequence}}\xspace}
\newcommand{\bvconsequences}{\ensuremath{\mathcal{BV}\mbox{-consequences}}\xspace}
\newcommand{\dpll}[1]{{\sc DPLL}\xspace}
\newcommand{\Atm}{{\ensuremath{\mathit{Atoms}}}}
\newcommand{\euf}{\ensuremath{\mathcal{EUF}}\xspace}
\newcommand{\arr}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\ee}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\dl}{\ensuremath{\mathcal{DL}}\xspace}
\newcommand{\la}{\ensuremath{\mathcal{LA}}\xspace}
\newcommand{\rat}{\ensuremath{\mathit{Rat}}\xspace}
\newcommand{\larat}{\ensuremath{\mathcal{LRA}}\xspace}
\newcommand{\laint}{\ensuremath{\mathcal{LIA}}\xspace}
\newcommand{\lia}{\ensuremath{\mathcal{LIA}}\xspace}
\newcommand{\mia}{\ensuremath{\mathcal{MIA}}\xspace}
\newcommand{\lra}{\ensuremath{\mathcal{LRA}}\xspace}
\newcommand{\Vars}[1]{{\ensuremath\mathit{Var}(#1)}}

\newcommand{\wordcast}[1]{{\wordcastsymb\texttt{(}#1\texttt{)}}}
\newcommand{\boolcast}[1]{{\texttt{bool(}#1\texttt{)}}}
\newcommand{\wordcastsymb}{\texttt{word1}}

\newcommand{\ITE}[3]{\ensuremath{\mbox{ITE}(#1, #2, #3)}}
\newcommand{\TITE}[3]{\ensuremath{\TITEsymb(#1, #2, #3)}}
\newcommand{\BITE}[3]{\ensuremath{\BITEsymb(#1, #2, #3)}}
\newcommand{\TITEsymb}{\ensuremath{\mbox{TITE}}\xspace}
\newcommand{\BITEsymb}{\ensuremath{\mbox{BITE}}\xspace}
\newcommand{\rew}{\ensuremath{\Rightarrow}}
\newcommand{\binconst}[1]{#1}
\newcommand{\vi}{{\ensuremath{\varphi}}\xspace}

\newcommand{\sm}[1]{SMT(#1)\xspace}

\newcommand{\floor}[1]{\ensuremath{\lfloor#1\rfloor}\xspace}

\newcommand{\LSHF}[1]{\ensuremath{\mbox{ LSH}(#1)}}
\newcommand{\RSHF}[1]{\ensuremath{\mbox{ RSH}(#1)}}
\newcommand{\AND}{\ensuremath{\mbox{ AND }}}
\newcommand{\OR}{\ensuremath{\mbox{ OR }}}
\newcommand{\XOR}{\ensuremath{\mbox{ XOR }}}
\newcommand{\NOT}{\ensuremath{\mbox{ NOT }}}
\newcommand{\ADDER}{\ensuremath{\mbox{ ADDER }}}
\newcommand{\MULT}[1]{\ensuremath{\mbox{ MULT}(#1)}}
\newcommand{\EQUAL}{\ensuremath{\mbox{ EQUAL }}}
\newcommand{\LEQ}{\ensuremath{\mbox{ LEQ }}}
\newcommand{\CONCAT}{\ensuremath{\mbox{ CONCAT }}}
\newcommand{\SELECT}[2]{\ensuremath{\mbox{ SELECT}[#1:#2]}}
\newcommand{\MUX}{\ensuremath{\mbox{ MUX }}}

\newcommand{\tracetolia}{\ensuremath{\eta}}

\newcommand{\irule}[2]{\ensuremath{#1 \ \| \ #2}}
\newcommand{\sep}{\ensuremath{\ | \ }}
\newcommand{\sepi}{\ensuremath{\rhd}\xspace}
\newcommand{\ifirule}[3]{\ensuremath{#1 \ \| \ #2 \ \mbox{ if } #3}}
\newcommand{\inA}[1]{\ensuremath{\lfloor #1 \rfloor_A}}
\newcommand{\inB}[1]{\ensuremath{\lfloor #1 \rfloor_B}}
\newcommand{\inX}[1]{\ensuremath{\lfloor #1 \rfloor_X}}

\newcommand{\normalize}[1]{\ensuremath{#1\downarrow}}
\newcommand{\rinfer}[3]{\ensuremath{\infer[#1]{#3}{#2}}}

\newcommand{\zchaff}{{\sc zChaff}\xspace}

\newcommand{\satsolver}{SAT-Solver\xspace}
\newcommand{\satsolvers}{SAT-Solvers\xspace}
\newcommand{\smtsolver}{SMT-Solver\xspace}
\newcommand{\smtsolvers}{SMT-Solvers\xspace}

\newcommand{\smteufut}{\ensuremath{SMT(\euf \cup \T)}}

\newcommand{\Lbrack}{\ensuremath{[\mspace{-3mu}[}}
\newcommand{\Rbrack}{\ensuremath{]\mspace{-3mu}]}}

\newcommand{\inter}[2]{\ensuremath{\Lbrack #1 \Rbrack^#2}}

\newcommand{\coarsest}[1]{\ensuremath{cs(#1)}}

\newcommand{\simp}[1]{\ensuremath{\sigma(#1)}}


\newcommand{\algfunc}{{\bf function}\xspace}
\newcommand{\algvar}{{\bf var}\xspace}
\newcommand{\algif}{{\bf if}\xspace}
\newcommand{\algforeach}{{\bf foreach}\xspace}
\newcommand{\algfor}{{\bf for}\xspace}
\newcommand{\algthen}{{\bf then}\xspace}
\newcommand{\algelse}{{\bf else}\xspace}
\newcommand{\algelseif}{{\bf elseif}\xspace}
\newcommand{\algend}{{\bf end}\xspace}
\newcommand{\algret}{{\bf return}\xspace}
\newcommand{\algand}{{\bf and}\xspace}
\newcommand{\algor}{{\bf or}\xspace}
\newcommand{\algwhile}{{\bf while}\xspace}

\newcommand{\pair}[2]{\ensuremath{\langle #1, #2 \rangle}}

\newcommand{\enode}{\emph{enode}\xspace}
\newcommand{\enodes}{\emph{enodes}\xspace}
\newcommand{\egraph}{\emph{egraph}\xspace}

\newcommand{\paper}[2]{#1}
\newcommand{\report}[2]{#2}

\newcommand{\footnoteremember}[2]
{
  \footnote{#2}
  \newcounter{#1}
  \setcounter{#1}{\value{footnote}}
}
\newcommand{\footnoterecall}[1]
{
  \footnotemark[\value{#1}]
}

\newcommand{\resolution}{\otimes}

\RequirePackage{color}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\COMMENT}[1]{}
\newcommand{\correction}[3][]{
  \sout{#2} \textcolor{red}{#3}
  \ifthenelse{\equal{#1}{}}{}{\footnote{#1}}
}
\newcommand{\lscomment}[1]{\textcolor{violet}{$\rangle\rangle$ LS : #1
    $\langle\langle$}}
\newcommand{\sgcomment}[1]{\textcolor{orange}{$\rangle\rangle$ SG : #1
    $\langle\langle$}}
\newcommand{\addition}[1]{\blue{#1}}


\newcommand{\ra}{\longrightarrow}
\newcommand{\lora}{\longrightarrow}
\newcommand{\alocal}{\ensuremath{A}-local\xspace}
\newcommand{\blocal}{\ensuremath{B}-local\xspace}
\newcommand{\astrict}{\ensuremath{A}-strict\xspace}
\newcommand{\bstrict}{\ensuremath{B}-strict\xspace}
\newcommand{\abcommon}{\ensuremath{AB}-common\xspace}
\newcommand{\abpure}{\ensuremath{AB}-pure\xspace}
\newcommand{\abmixed}{\ensuremath{AB}-mixed\xspace}
\newcommand{\st}{\; \vert \;}
\newcommand{\idx}[2][i]{\ensuremath {#1 \in \{1,\ldots,\mbox{$#2$}\}}}
\newcommand{\ual}{\ensuremath{\underline {\alpha}}}
\newcommand{\ube}{\ensuremath{\underline {\beta}}}
\newcommand{\ua}{\ensuremath{\underline a}}
\newcommand{\ub}{\ensuremath{\underline b}}
\newcommand{\uc}{\ensuremath{\underline c}}
\newcommand{\ud}{\ensuremath{\underline d}}
\newcommand{\ue}{\ensuremath{\underline e}}
\newcommand{\ug}{\ensuremath{\underline g}}
\newcommand{\uh}{\ensuremath{\underline h}}
\newcommand{\ui}{\ensuremath{\underline i}}
\newcommand{\uj}{\ensuremath{\underline j}}
\newcommand{\uk}{\ensuremath{\underline k}}
\newcommand{\ut}{\ensuremath{\underline t}}
\newcommand{\ux}{\ensuremath{\underline x}}
\newcommand{\uu}{\ensuremath{\underline u}}
\newcommand{\uU}{\ensuremath{\underline U}}
\newcommand{\uF}{\ensuremath{\underline F}}
\newcommand{\uH}{\ensuremath{\underline H}}
\newcommand{\uy}{\ensuremath{\underline y}}
\newcommand{\uz}{\ensuremath{\underline z}}
\newcommand{\us}{\ensuremath{\underline s}}
\newcommand{\ul}{\ensuremath{\underline l}}
\newcommand{\up}{\ensuremath{\underline p}}
\newcommand{\cA}{\ensuremath \mathcal A}
\newcommand{\cB}{\ensuremath \mathcal B}
\newcommand{\cM}{\ensuremath \mathcal M}
\newcommand{\cN}{\ensuremath \mathcal N}
\newcommand{\cT}{\ensuremath \mathcal T}
\newcommand{\cS}{\ensuremath \mathcal S}
\newcommand{\cC}{\ensuremath \mathcal C}
\newcommand{\cL}{\ensuremath \mathcal L}
\newcommand{\cV}{\ensuremath \mathcal V}
\newcommand{\cP}{\ensuremath \mathcal P}
\newcommand{\cF}{\ensuremath \mathcal F}
\newcommand{\cI}{\ensuremath \mathcal I}
\newcommand{\cJ}{\ensuremath \mathcal J}

\newcommand{\val}[1]{\ensuremath #1_{\cM, \cI}}
\newcommand{\valp}[1]{\ensuremath #1_{\cM, \cI'}}

\newcommand{\Proc}{\ensuremath \mathtt{Proc}}
\newcommand{\Data}{\ensuremath \mathtt{Data}}

\newcommand{\aze}{\ensuremath T^I_E}
\newcommand{\lnext}{\ensuremath X}
\newcommand{\lbox}{\ensuremath \Box}
\newcommand{\ldiamond}{\ensuremath \Diamond}
\newcommand{\luntil}{\ensuremath U}
\newcommand{\lrelease}{\ensuremath R}
\newcommand{\ltl}{LTL}
\newcommand{\ltlt}{\ltl(\ensuremath {\mathcal T})}
\newcommand{\dpllt}{\textit{DPLL}(\ensuremath {\mathcal T})}
\newcommand{\ltlfor}{\ltl($\Sigma^{\ua}$)}
\newcommand{\ltlforci}{\ltl($\Sigma^{\uc}$)}
\newcommand{\ltlforc}{\ltl($\Sigma^{\ua, \uc}$)}
\newcommand{\abstr}[1][\varphi]{\ensuremath {\lbrack\!\lbrack\, #1 \,\rbrack\!\rbrack}}
\renewcommand{\int}{\ensuremath {\mathcal I}}
\newcommand{\closure}{\ensuremath {cl}}
\newcommand{\pre}[1][T]{\ensuremath {Res_{#1}}}
\newcommand{\disjcup}{\ensuremath \oplus}
\newcommand{\bigdisjcup}{\ensuremath \bigoplus}
\newcommand{\sysset}{\ensuremath {\langle \Sigma, T, \Sigma_r, \ua, \uc \rangle}}
\newcommand{\sysspec}{\ensuremath {(\mathcal T, \delta, \iota)}}
\newcommand{\satproc}{\textit{``satisfiable''}}
\newcommand{\unsatproc}{\textit{``unsatisfiable''}}
\newcommand{\prename}{residue enumerator}
\newcommand{\pbename}{\prename}
\newcommand{\secname}{Section~}
\newcommand{\theory}{dataflow theory}
\newcommand{\theories}{dataflow theories}
\renewcommand{\sp}{\ensuremath{\mathcal{SP}}}
\newcommand{\Tcon}{$T$-constraint\ }
\newcommand{\Tcons}{$T$-constraints\ }
\newcommand{\mywidehat}[1]{\ensuremath{\lbrack\!\lbrack #1 \rbrack\!\rbrack}}
\newcommand{\myparagraph}[1]{\noindent \textbf{#1}}
\newcommand{\rbcomment}[1]{\textcolor{blue}{[RB: #1]}}
\newcommand{\facomment}[1]{\textcolor{cyan}{[FA: #1]}}
\newcommand{\srcomment}[1]{\textcolor{red}{[SR: #1]}}
\newcommand{\nscomment}[1]{\textcolor{black}{[NS: #1]}}
\newcommand{\algoname}{Algorithm}

\newcommand{\sindex}{\ensuremath{{\tt INDEX}}\xspace}
\newcommand{\sint}{\ensuremath{{\tt INT}}\xspace}
\newcommand{\sarray}{\ensuremath{{\tt ARRAY}}\xspace}
\newcommand{\sarrayl}{\ensuremath{{\tt ARRAY}_{\ell}}\xspace}
\newcommand{\sarraylh}{\ensuremath{{\tt ARRAY}_{\ell_h}}\xspace}
\newcommand{\sarraylk}{\ensuremath{{\tt ARRAY}_{\ell_k}}\xspace}
\newcommand{\selem}{\ensuremath{{\tt ELEM}}\xspace}
\newcommand{\seleml}{\ensuremath{{\tt ELEM}_{\ell}}\xspace}
\newcommand{\selemlp}{\ensuremath{{\tt ELEM}_{\ell'}}\xspace}

\def\Examplesize{\fontsize{8pt}{8pt}\selectfont}


\newcommand{\ta}{\ensuremath{{\bf a}}\xspace}
\newcommand{\tc}{\ensuremath{{\bf c}}\xspace}
\newcommand{\td}{\ensuremath{{\bf d}}\xspace}
\newcommand{\tv}{\ensuremath{{\bf v}}\xspace}
\newcommand{\tb}{\ensuremath{{\bf b}}\xspace}
\newcommand{\tk}{\ensuremath{{\bf k}}\xspace}
\newcommand{\tf}{\ensuremath{{\bf f}}\xspace}
\newcommand{\tte}{\ensuremath{{\bf e}}\xspace}
\newcommand{\tr}{\ensuremath{{\bf r}}\xspace}
\newcommand{\tts}{\ensuremath{{\bf s}}\xspace}
\newcommand{\tw}{\ensuremath{{\bf w}}\xspace}
\newcommand{\tu}{\ensuremath{{\bf u}}\xspace}
\newcommand{\ttb}{\ensuremath{{\bf t}}\xspace}
\newcommand{\tU}{\ensuremath{{\bf U}}\xspace}
\newcommand{\tF}{\ensuremath{{\bf F}}\xspace}
\newcommand{\tH}{\ensuremath{{\bf H}}\xspace}
\newcommand{\ti}{\ensuremath{{\bf i}}\xspace}
\newcommand{\tx}{\ensuremath{{\bf x}}\xspace}
\newcommand{\tz}{\ensuremath{{\bf z}}\xspace}
\newcommand{\tM}{\ensuremath{{\bf M}}\xspace}

\newcommand{\fakeparagraph}[1]{\\\noindent{\em #1}}

\newcommand{\pres}{\ensuremath{{\mathbb P}}\xspace}
\newcommand{\ARR}{\ensuremath{{\mathtt{ARR}}}\xspace}

\newcommand{\set}[1]{\{\, #1 \,\}}
\newcommand{\card}{\mathrm{card}}
\newcommand{\length}[1]{|#1|}
\newcommand{\rto}{\xrightarrow{\;\;}}
\newcommand{\Pz}{\mathrm{P}_{0}}
\newcommand{\Jz}{\mathrm{J}_{0}}
\newcommand{\chiS}{\chi^{S}}
\newcommand{\Schi}{S_{\chi}}
\newcommand{\tiff}{\quad\text{iff}\quad}
\newcommand{\downset}{\downarrow}
\newcommand{\chiStar}{\chi^{-1}}
\newcommand{\Chi}[1]{\overline{#1}}

\newcommand{\core}{\mathrm{core}}
\newcommand{\pairOfTypes}[2]{\binom{#1}{#2}}
\newcommand{\typeOfP}[2]{\binom{#1}{#2}}
\newcommand{\hheight}{\mathrm{height}}
\newcommand{\ddownset}{\downarrow\!\!\downarrow}

\newcommand{\cl}[1]{[#1]_{n-1}}
\newcommand{\iCl}[1]{[#1]^\mathtt{2}_{n-1}}
\newcommand{\types}{\mathtt{ty}_{\tiny n-1}}
\newcommand{\ty}{\types}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\Stypes}{\mathtt{t}}
\newcommand{\sty}{\Stypes}
\newcommand{\vu}[1][]{(v,u)^{#1}}
\newcommand{\Chivu}{\Chi{\vu}}
\newcommand{\nvu}{\psi(v,u)}
\newcommand{\Chinvu}{\Chi{\nvu}}
\newcommand{\nnvu}{(v,\Chinvu)}
\newcommand{\Chinnvu}{\Chi{\nnvu}}
\newcommand{\Svu}{S_{\vu}}
\newcommand{\Rvu}{R_{\vu}}
\newcommand{\pz}{p_{0}}
\newcommand{\Periodic}[1]{\Pi_{#1}}
\newcommand{\Pvu}{\Pi_{\vu}}
\newcommand{\Pnvu}{\Pi_{\nvu}}


\newcommand{\smalleql}[1]{\makebox[2cm][l]{$\displaystyle{#1}$}}

\newcommand{\fp}{finitely-presented\xspace}

\newcommand{\GRZL}{Grzegorczyk's Logic\xspace}
\newcommand{\grzl}{\GRZL}

\newcommand{\modified}[3][]{
  \blue{#3}
  \footnote{
    Original : \red{#2}\\
    \ifthenelse{\equal{#1}{}}{}
    {Comment: #1}
  }
}

\newcommand{\FH}[2][H]{#1(#2)}

\newcommand{\eqdef}{:=}


\newenvironment{fact*}{\par\smallskip\noindent{\em
    Fact.}~\em}{\smallskip}
\newcommand{\RT}{Ruitenburg's Theorem\xspace}
\newcommand{\mcd}{\mathrm{mcd}}
\newcommand{\mcm}{\mathrm{mcm}}
\newcommand{\lcm}{\mathrm{lcm}}
\newcommand{\nonperiodic}{non-periodic\xspace}
\newcommand{\Eper}{E_{per}}
\newcommand{\Rho}[1]{\rho(#1)}
\newcommand{\Pzero}{{\bf P}_{\bf 0}}
\newcommand{\PzeroOp}{\Pzero^{op}}


